Analyzing Political Parody in Social Media

Parody is a figurative device used to imitate an entity for comedic or critical purposes and represents a widespread phenomenon in social media through many popular parody accounts. In this paper, we present the first computational study of parody. We introduce a new publicly available data set of tweets from real politicians and their corresponding parody accounts. We run a battery of supervised machine learning models for automatically detecting parody tweets with an emphasis on robustness by testing on tweets from accounts unseen in training, across different genders and across countries. Our results show that political parody tweets can be predicted with an accuracy up to 90%. Finally, we identify the markers of parody through a linguistic analysis. Beyond research in linguistics and political communication, accurately and automatically detecting parody is important to improving fact checking for journalists and analytics such as sentiment analysis through filtering out parodical utterances.

==> result_tables_full_notused.tex <==

%%%%%%%%%%%%%%%%%%%% GENDER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% trained on FEMALE
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |l|l|l|l|l|}
\cellcolor[HTML]{C0C0C0}\textbf{Model} & \cellcolor[HTML]{C0C0C0}\textbf{Accuracy} & \cellcolor[HTML]{C0C0C0}\textbf{Precision} & \cellcolor[HTML]{C0C0C0}\textbf{Recall} & \cellcolor[HTML]{C0C0C0}\textbf{F1-Score} & \cellcolor[HTML]{C0C0C0}\textbf{AUC} \\ \toprule
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Logistic Regression}                                                                                                                                                                                            \\
Unigrams                               & 75.63 ($\pm$ 0.001)                            & 74.00 ($\pm$ 0.003)                             & 79.46 ($\pm$ 0.006)                          & 76.63 ($\pm$ 0.002)                            & 75.61 ($\pm$ 0.001)                       \\
POS Trigram                            & 75.88 ($\pm$ 0.001)                            & 74.50 ($\pm$ 0.003)                             & 79.12 ($\pm$ 0.003)                          & 76.74 ($\pm$ 0.000)                            & 75.86 ($\pm$ 0.001)                       \\
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Neural Network}                                                                                                                                                                                                 \\
LSTM                                   & 74.97 ($\pm$ 0.009)                            & 78.52 ($\pm$ 0.034)                             & 69.83 ($\pm$ 0.068)                          & 73.55 ($\pm$ 0.027)                            & 75.00 ($\pm$ 0.009)                       \\
Bi-LSTM                                & 75.03 ($\pm$ 0.006)                            & 79.11 ($\pm$ 0.031)                             & 68.97 ($\pm$ 0.059)                          & 73.41 ($\pm$ 0.020)                            & 75.06 ($\pm$ 0.006)                       \\
Bi-LSTM-Att                            & 74.90 ($\pm$ 0.013)                            & 78.98 ($\pm$ 0.030)                             & 68.83 ($\pm$ 0.069)                          & 73.20 ($\pm$ 0.031)                            & 74.93 ($\pm$ 0.013)                       \\
BERT                                   & 83.41 ($\pm$ 0.399)                            & 89.25 ($\pm$ 0.393)                             & 80.05 ($\pm$ 0.385)                          & 84.40 ($\pm$ 0.355)                            & 83.37 ($\pm$ 0.392)                       \\
RoBERTa                                & \textbf{83.98 ($\pm$ 0.346)}                   & \textbf{89.32 ($\pm$ 0.324)}                    & \textbf{84.87 ($\pm$ 0.362)}                 & \textbf{84.87 ($\pm$ 0.388)}                   & \textbf{83.95 ($\pm$ 0.385)}              \\
XLNet                             & 83.29 ($\pm$ 0.376)                            & 88.27 ($\pm$ 0.375)                             & 80.42 ($\pm$ 0.391)                          & 84.16 ($\pm$ 0.361)                            & 83.26 ($\pm$ 0.382)                       \\
ULMFit                                 & 81.64 ($\pm$ 0.546)                            & 79.13 ($\pm$ 0.573)                             & 86.23 ($\pm$ 0.481)                          & 82.53 ($\pm$ 0.543)                            & 81.62 ($\pm$ 0.468)     \\ \bottomrule                 
\end{tabular}
}
\caption{Parody prediction results using logistic regression and neural network approaches on the gender split dataset trained on the female subgroup. Best results are in bold}
\label{tab:resultsfemale}
\end{table*}


% trained on MALE
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |l|l|l|l|l|}
\cellcolor[HTML]{C0C0C0}\textbf{Model} & \cellcolor[HTML]{C0C0C0}\textbf{Accuracy} & \cellcolor[HTML]{C0C0C0}\textbf{Precision} & \cellcolor[HTML]{C0C0C0}\textbf{Recall} & \cellcolor[HTML]{C0C0C0}\textbf{F1-Score} & \cellcolor[HTML]{C0C0C0}\textbf{AUC} \\ \toprule
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Logistic Regression}       
\\ 
LR Bigrams                             & 78.42 ($\pm$ 0.000)                            & 74.31 ($\pm$ 0.000)                             & 84.06 ($\pm$ 0.001)                          & 78.89 ($\pm$ 0.000)                            & 78.64 ($\pm$ 0.000)                       \\ \hline
LR POS Trigrams                        & 78.08 ($\pm$ 0.000)                            & 73.64 ($\pm$ 0.001)                             & 84.59 ($\pm$ 0.001)                          & 78.74 ($\pm$ 0.000)                            & 78.34 ($\pm$ 0.000)                       \\ \hline
\multicolumn{6}{l}{\cellcolor[HTML]{C0C0C0}Neural Networks}                                                                                                                                                                                                  \\ \hline
LSTM                                   & 77.92 ($\pm$ 0.010)                            & 82.24 ($\pm$ 0.028)                             & 69.23 ($\pm$ 0.056)                          & 74.92 ($\pm$ 0.026)                            & 77.58 ($\pm$ 0.012)                       \\ \hline
Bi-LSTM                                & 78.49 ($\pm$ 0.005)                            & 80.07 ($\pm$ 0.008)                             & 73.47 ($\pm$ 0.014)                          & 76.62 ($\pm$ 0.006)                            & 78.30 ($\pm$ 0.005)                       \\ \hline
Bi-LSTM-Att                            & 78.09 ($\pm$ 0.005)                            & 83.17 ($\pm$ 0.028)                             & 68.45 ($\pm$ 0.045)                          & 74.91 ($\pm$ 0.016)                            & 77.71 ($\pm$ 0.006)                       \\ \hline
BERT                                   & 86.80 ($\pm$ 0.318)                            & 83.45 ($\pm$ 0.390)                             & 88.38 ($\pm$ 0.387)                          & 85.85 ($\pm$ 0.288)                            & 86.67 ($\pm$ 0.334)                       \\ \hline
RoBERTa                                & \textbf{87.68 ($\pm$ 0.343)}                   & \textbf{86.86 ($\pm$ 0.405)}                    & \textbf{87.37 ($\pm$ 0.371)}                 & \textbf{87.11 ($\pm$ 0.316)}                   & \textbf{87.64 ($\pm$ 0.355)}              \\ \hline
XLNet                             & 86.64 ($\pm$ 0.345)                            & 83.38 ($\pm$ 0.366)                             & 88.13 ($\pm$ 0.399)                          & 85.69 ($\pm$ 0.257)                            & 86.51 ($\pm$ 0.301)                       \\ \hline
ULMFit                                 & 82.93 ($\pm$ 0.321)                            & 86.05 ($\pm$ 0.289)                             & 76.88 ($\pm$ 0.295)                          & 81.20 ($\pm$ 0.286)                            & 82.69 ($\pm$ 0.324)                       \\ \bottomrule
\end{tabular}
}
\caption{Parody prediction results using logistic regression and neural network approaches on the gender split dataset trained on the male subgroup. Best results are in bold}
\label{tab:resultsmale}
\end{table*}


































%%%%%%%%%%%%%%%%%%%% LOCATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%% UK Intl
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}\textbf{Model}} & \cellcolor[HTML]{C0C0C0}\textbf{Accuracy} & \cellcolor[HTML]{C0C0C0}\textbf{Precision} & \cellcolor[HTML]{C0C0C0}\textbf{Recall} & \cellcolor[HTML]{C0C0C0}\textbf{F1-Score} & \cellcolor[HTML]{C0C0C0}\textbf{AUC} \\ \toprule
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Logistic Regression}                                                                                                                                                                                                                  \\ \hline
Trigrams                                                     & 77.93 ($\pm$0.001)                            & 77.80 ($\pm$0.003)                             & 75.99 ($\pm$0.004)                          & 77.97 ($\pm$0.001)                            & 77.99 ($\pm$0.001)                       \\ \hline
POS Bigrams                                                  & 77.80 ($\pm$0.001)                            & 75.84 ($\pm$0.002)                             & 76.95 ($\pm$0.005)                          & 78.08 ($\pm$0.002)                            & 77.82 ($\pm$0.001)                       \\ \hline
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Neural Networks}                                                                                                                                                                                                                      \\ \hline
LSTM                                                         & 80.47 ($\pm$0.007)                            & 80.47 ($\pm$0.024)                             & 79.33 ($\pm$0.026)                          & 79.84 ($\pm$0.007)                            & 80.44 ($\pm$0.007)                       \\ \hline
LSTM                                                         & 75.84 ($\pm$0.013)                            & 76.29 ($\pm$0.018)                             & 63.14 ($\pm$0.047)                          & 72.77 ($\pm$0.026)                            & 76.20 ($\pm$0.012)                       \\ \hline
Bi-LSTM                                                      & 76.29 ($\pm$0.009)                            & 75.92 ($\pm$0.027)                             & 66.02 ($\pm$0.049)                          & 74.01 ($\pm$0.022)                            & 76.59 ($\pm$0.008)                       \\ \hline
Bi-LSTM-Att                                                  & 75.92 ($\pm$0.011)                            & 84.11 ($\pm$0.018)                             & 64.27 ($\pm$0.045)                          & 73.19 ($\pm$0.023)                            & 76.25 ($\pm$0.010)                       \\ \hline
BERT                                                         & 84.11 ($\pm$0.513)                            & 86.26 ($\pm$1.142)                             & 91.59 ($\pm$0.951)                          & 83.12 ($\pm$0.607)                            & 84.34 ($\pm$0.562)                       \\ \hline
RoBERTa                                                      & \textbf{86.26 ($\pm$0.602)}                   & \textbf{84.23 ($\pm$0.789)}                    & \textbf{90.32 ($\pm$0.427)}                 & \textbf{85.99 ($\pm$0.612)}                   & \textbf{86.38 ($\pm$0.471)}              \\ \hline
XLNet                                                   & 85.22 ($\pm$0.511)                            & 83.55 ($\pm$0.912)                             & 87.16 ($\pm$0.650)                          & 85.36 ($\pm$0.538)                            & 85.27 ($\pm$0.493)                       \\ \hline
ULMFit                                                       & 82.60 ($\pm$1.167)                            & 79.30 ($\pm$1.122)                             & 83.92 ($\pm$1.008)                          & 81.55 ($\pm$0.966)                            & 82.50 ($\pm$0.928)                       \\ \bottomrule
\end{tabular}
}
\caption{Parody prediction results using logistic regression and neural network approaches on the location split dataset trained on the UK \& Other subgroup. Best results are in bold}
\label{tab:resultsukIntl}
\end{table*}


%US UK

\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |c|c|c|c|c|}
\hline
\cellcolor[HTML]{C0C0C0}\textbf{Model} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Accuracy}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Precision}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Recall}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{F1-Score}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{AUC}} \\ \toprule
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Logistic Regression}                                                                                                                                                                                                                                                                                                     \\ \hline
LR Trigrams                            & 76.98 ($\pm$0.001)                                                 & 71.98 ($\pm$0.002)                                                  & 86.48 ($\pm$0.003)                                               & 78.57 ($\pm$0.000)                                                 & 77.21 ($\pm$0.001)                                            \\ \hline
LR POS Trigrams                        & 76.48 ($\pm$0.000)                                                 & 71.24 ($\pm$0.001)                                                  & 86.85 ($\pm$0.001)                                               & 78.27 ($\pm$0.000)                                                 & 76.73 ($\pm$0.000)                                            \\ \hline
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Neural Networks}                                                                                                                                                                                                                                                                                                         \\ \hline
LSTM                                   & 80.47 ($\pm$0.007)                                                 & 80.51 ($\pm$0.024)                                                  & 79.33 ($\pm$0.026)                                               & 79.84 ($\pm$0.007)                                                 & 80.44 ($\pm$0.007)                                            \\ \hline
Bi-LSTM                                & 80.06 ($\pm$0.011)                                                 & 78.78 ($\pm$0.029)                                                  & 81.29 ($\pm$0.030)                                               & 79.91 ($\pm$0.006)                                                 & 80.09 ($\pm$0.010)                                            \\ \hline
Bi-LSTM-Att                            & 81.02 ($\pm$0.008)                                                 & 81.29 ($\pm$0.014)                                                  & 79.47 ($\pm$0.036)                                               & 80.29 ($\pm$0.013)                                                 & 80.98 ($\pm$0.008)                                            \\ \hline
BERT                                   & 86.19 ($\pm$0.303)                                                 & \textbf{92.10 ($\pm$0.278)}                                                  & 81.87 ($\pm$0.364)                                               & 86.69 ($\pm$0.457)                                                 & 86.33 ($\pm$0.372)                                            \\ \hline
RoBERTa                                & \textbf{87.45 ($\pm$0.294)}                                        & 91.69 ($\pm$0.344)                                         & \textbf{84.04 ($\pm$0.401)}                                      & \textbf{87.70 ($\pm$0.452)}                                        & \textbf{87.55 ($\pm$0.388)}                                   \\ \hline
XLNet                             & 84.58 ($\pm$0.322)                                                 & 91.83 ($\pm$0.236)                                                  & 79.67 ($\pm$0.357)                                               & 85.32 ($\pm$0.418)                                                 & 84.74 ($\pm$0.358)                                            \\ \hline
ULMFit                                 & 83.08 ($\pm$0.339)                                                 & 79.70 ($\pm$0.489)                                                  & 87.62 ($\pm$0.355)                                               & 83.47 ($\pm$0.391)                                                 & 83.18 ($\pm$0.376)                                            \\ \bottomrule
\end{tabular}
}
\caption{Parody prediction results using logistic regression and neural network approaches on the location split dataset trained on the US \& UK  subgroup. Best results are in bold}
\label{tab:resultsUSUK}

\end{table*}



% US Intl
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |c|c|c|c|c|}
\hline
\cellcolor[HTML]{C0C0C0}\textbf{Model} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Accuracy}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Precision}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{Recall}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{F1-Score}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\textbf{AUC}} \\ \hline
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} Logistic Regression}}                                                                                                                                                                                                                                                                              \\ \hline
Trigrams                               & 78.51 ($\pm$0.000)                                                 & 76.79 ($\pm$0.001)                                                  & 79.82 ($\pm$0.002)                                               & 78.27 ($\pm$0.000)                                                 & 78.55 ($\pm$0.000)                                            \\ \hline
POS Trigrams                           & 77.93 ($\pm$0.000)                                                 & 75.76 ($\pm$0.001)                                                  & 80.13 ($\pm$0.001)                                               & 77.88 ($\pm$0.000)                                                 & 77.99 ($\pm$0.000)                                            \\ \hline
\multicolumn{6}{|l|}{\cellcolor[HTML]{C0C0C0}Neural Networks}                                                                                                                                                                                                                                                                                                         \\ \hline
LSTM                                   & 80.47 ($\pm$0.007)                                                 & 84.61 ($\pm$0.018)                                                  & 69.33 ($\pm$0.034)                                               & 76.12 ($\pm$0.014)                                                 & 78.67 ($\pm$0.006)                                            \\ \hline
LSTM                                   & 78.96 ($\pm$0.005)                                                 & 84.61 ($\pm$0.018)                                                  & 69.33 ($\pm$0.034)                                               & 76.12 ($\pm$0.014)                                                 & 78.67 ($\pm$0.006)                                            \\ \hline
Bi-LSTM                                & 79.23 ($\pm$0.003)                                                 & 84.00 ($\pm$0.007)                                                  & 70.65 ($\pm$0.017)                                               & 76.73 ($\pm$0.007)                                                 & 78.98 ($\pm$0.004)                                            \\ \hline
Bi-LSTM-Att                            & 79.22 ($\pm$0.005)                                                 & 82.56 ($\pm$0.020)                                                  & 72.68 ($\pm$0.038)                                               & 77.19 ($\pm$0.013)                                                 & 79.03 ($\pm$0.006)                                            \\ \hline
BERT                                   & 84.96 ($\pm$0.223)                                                 & 80.11 ($\pm$0.258)                                                  & 87.80 ($\pm$0.231)                                               & 83.78 ($\pm$0.198)                                                 & 84.82 ($\pm$0.256)                                            \\ \hline
RoBERTa                                & \textbf{85.83 ($\pm$0.304)}                                        & 83.44 ($\pm$0.315)                                         & \textbf{86.82 ($\pm$0.313)}                                      & 85.10 ($\pm$0.278)                                        & \textbf{85.76 ($\pm$0.294)}                                   \\ \hline
XLNet                             & 85.41 ($\pm$0.289)                                                 & \textbf{86.37 ($\pm$0.328)}                                                  & 84.00 ($\pm$0.346)                                               & \textbf{85.17 ($\pm$0.293)}                                                 & 85.44 ($\pm$0.352)                                            \\ \hline
ULMFit                                 & 82.60 ($\pm$0.785)                                                 & 79.30 ($\pm$0.306)                                                  & 83.92 ($\pm$0.398)                                               & 81.55 ($\pm$0.505)                                                 & 82.50 ($\pm$0.613)                                            \\ \hline
\end{tabular}
}
\caption{Parody prediction results using logistic regression and neural network approaches on the location split dataset trained on the US \& Other subgroup. Best results are in bold}
\label{tab:resultsUSIntl}
\end{table*}

